Training Dynamic Exponential Family Models with Causal and Lateral Dependencies for Generalized Neuromorphic Computing

Neuromorphic hardware platforms, such as Intel's Loihi chip, support the implementation of Spiking Neural Networks (SNNs) as an energy-efficient alternative to Artificial Neural Networks (ANNs). SNNs are networks of neurons with internal analogue dynamics that communicate by means of binary time series. In this work, a probabilistic model is introduced for a generalized set-up in which the synaptic time series can take values in an arbitrary alphabet and are characterized by both causal and instantaneous statistical dependencies. The model, which can be considered as an extension of exponential family harmoniums to time series, is introduced by means of a hybrid directed-undirected graphical representation. Furthermore, distributed learning rules are derived for Maximum Likelihood and Bayesian criteria under the assumption of fully observed time series in the training set.

==> model_old.tex <==
\section{Models for Probabilistic SNNs}

\subsection{Directed Models}

Here we can write the main equations that define directed information graphs and explain the main modeling equations. You may refer to the attached "text" document (with accompanying "reference" file). Please note that the text was written assuming a Poisson distribution, but we should change it to {\em Bernoulli} variables as done in Alireza's paper for a two-layer network. As in Alireza's paper, let us allow for a parametrization in terms of generic basis functions.

Directed models account for causality relationships between the operations of neurons in space and time. They are easy to sample from via ancestral sampling. They may account for rate and time encoding / decoding, but population encoding is more difficult to model given the conditional independence of current outputs given previous values of the spiking outputs. 

\vspace{3cm}

\newpage
\subsection{Undirected Models}

Please see my handwritten notes. It seems to me that we can define undirected models that capture the instantaneous "affinity" between the outputs of different neurons. This makes it possible to capture population coding as in, e.g., the Winner-Take-All circuit. Again, we should write main equations and mention the use of generic basis functions.

\vspace{1cm}

\newpage 
\subsection{Supervised and Unsupervised Learning for Exponential Family Harmoniums for Time-series with Applications to Spiking Neural Networks}

\smallskip
$\circ$ Notations.

\begin{enumerate}
\item $N_x, N_h$: number of visible and hidden unit or neurons

\smallskip
\item Bipartite topology for each time instant: one visible layer and one hidden layer with no inside-layer connections.

\smallskip
\item $x_i, h_j$: visible unit $i = 1, \cdots, N_x$ and hidden unit $j = 1, \cdots, N_h$ can take values in either the continuous or the discrete domain.

\smallskip
\item $\bfx_t := [x_{1,t}, \cdots, x_{i,t}, \cdots, x_{N_x,t}]^\top, \bfh_t := [h_{1,t}, \cdots, h_{j,t},\cdots, h_{N_h,t}]^\top$ is visible and hidden vector at time $t$, respectively. (column vector: $N_x \times 1$, $N_h \times 1$ vector)

\smallskip
\item $\bfx^{t} := (\bfx_0, \bfx_1, \cdots, \bfx_t ), \bfh^{t} = (\bfh_0,\cdots, \bfh_t)$: time-series data from time $0$ to $t$ of visible and hidden, respectively.

\smallskip
\item $\bfs_i(x_i) := [s_{i,1}(x_i), \cdots, s_{i,a}(x_i), \cdots, s_{i,N_a}(x_i)]^\top, \bfz_j(h_j) := [z_{j,1}(h_j), \cdots, z_{j,b}(h_j), \cdots, z_{j,N_b}(h_j)]^\top$: $N_a$ dimensional sufficient statistics of visible unit $i$ and $N_b$ dimensional hidden unit $j$, respectively. $a$ is an index for sufficient statistic of visible unit and $b$ is an index for one of hidden unit. For simplicity, we denote by $\bfs_{i,t} := \bfs_i(x_{i,t})$ the sufficient statistics of visible unit $i$ at time $t$. Similarly, we use $\bfz_{j,t} := \bfz_j(h_{j,t})$. $\bfs_{i,t}$ is $N_a \times 1$ column vector and $\bfz_{j,t}$ is $N_b \times 1$ column vector

\smallskip
\item Joint probability distribution:
\begin{align} \label{eq:EFH-joint}
p(\bfx_t,\bfh_t | \bfx^{t-1},\bfh^{t-1}) \propto \exp \bigg\{ 
& \sum_{i} \bmtheta_i^\top \bfs_{i,t} + \sum_{j} \bmlambda_j^\top \bfz_{j,t} + \sum_{i,j} \bfs_{i,t}^\top \bfU_{i,j} \bfz_{j,t} \cr 
& + \sum_{\delta=1}^\tau \Big( \sum_{i',i} \bfs_{i',t-\delta}^\top \bfW_{i',i}^{[\delta]} \bfs_{i,t} + \sum_{j',i} \bfz_{j',t-\delta}^\top \bfW_{j',i}^{[\delta]} \bfs_{i,t} \cr 
& \qquad \qquad + \sum_{i',j} \bfs_{i',t-\delta}^\top \bfW_{i',j}^{[\delta]} \bfz_{j,t} + \sum_{j',j} \bfz_{j',t-\delta}^\top \bfW_{j',j}^{[\delta]} \bfz_{j,t} \Big)
\bigg\}
\end{align}
\begin{comment}
Simply, Let denote by followings: (i) $\bfs_t := [\bfs_{1,t}^\top, \cdots, \bfs_{i,t}^\top, \cdots, \bfs_{N_x,t}^\top]^\top = [\bfs_{1,t}; \cdots ; \bfs_{i,t}; \cdots; \bfs_{N_x,t}]$ is $N_x \cdot N_a$ column vector, (ii) $\bfW^{[\delta]} := [\bfW_{i,j}]$ is $N_x \cdot N_a \times N_h \cdot N_b$ matrix, (iii) $\bfz_t := [\bfz_{1,t}^\top, \cdots, \bfz_{j,t}^\top, \cdots, \bfz_{N_h,t}^\top]^\top = [\bfz_{1,t}; \cdots; \bfz_{j,t}; \cdots; \bfz_{N_h,t}]$ is $N_h \cdot N_b$ column vector, then $\sum_{i',j} \bfs_{i',t-\delta}^\top \bfW_{i',j}^{[\delta]} \bfz_{j,t} = \bfs_{t-\delta}^\top \bfW^{[\delta]} \bfz_{t}$
\end{comement}

\begin{comment}
\begin{align}
p(\bfx_t,\bfh_t | \bfx^{t-1},\bfh^{t-1}) \propto \exp \bigg\{ 
& \sum_{i} \bmth_i^\top \bfs_{i,t} + \sum_{j} \bml_j^\top \bfz_{j,t} + \sum_{i,j} \bfs_{i,t}^\top \bfU_{i,j} \bfz_{j,t} \cr 
& + \sum_{\delta=1}^\tau \left[ [\bfs_{i,t-\delta}^\top]_{i=1,\cdots,N_x}, [\bfz_{j,t-\delta}^\top]_{j=1,\cdots,N_h} \right] \bfW^{[\delta]} \cr 
& \qquad \qquad \left[ [\bfs_{i,t}^\top]_{i=1,\cdots,N_x}, [\bfz_{j,t}^\top]_{j=1,\cdots,N_h} \right]^\top
\bigg\}
\end{align}
\end{comment}

\smallskip
\item $\bmtheta_i := [\theta_{i,1}, \cdots, \theta_{i,a},\cdots, \theta_{i,N_a}]^\top, \bmlambda_j := [\lambda_{j,1},\cdots,\lambda_{j,b},\cdots,\lambda_{j,N_b}]^\top$: singleton parameter of visible unit $i$ and hidden unit $j$. (column vectors: $N_a \times 1, N_b \times 1$)
%Simply, $\bmth = [\bmth_1, \cdots, \bmth_i, \cdots, \bmth_{N_x}]^\top$(??) and $\bml = [\bml_1, \cdots, \bml_j, \cdots, \bml_{N_h}]^\top$.

\smallskip
\item $\bfU := [\bfU_{i,j}]_{i,j}$ where $\bfU_{i,j}$ is $N_a \times N_b$ matrix whose element is {\em instantaneous} interaction parameter between $a$-th sufficient statistics of visible unit $i$ and $b$-th sufficient statistics of hidden unit $j$. 

\smallskip
\item For every $\delta \in [1,\tau]$, for all $i,i' = 1, \cdots, N_x$ and $j,j' = 1, \cdots, N_h$, we have followings: $\bfW_{i',i}^{[\delta]}$ is $N_a \times N_a$ matrix, $\bfW_{i',j}^{[\delta]}$ is $N_a \times N_b$ matrix, $\bfw_{j',i}^{[\delta]}$ is $N_b \times N_a$ matrix, and $\bfW_{j',j}^{[\delta]}$ is $N_b \times N_b$ matrix. In particular, $\bfW_{i',i}^{[\delta]} = [w_{i'a',ia}^{[\delta]}]_{N_a \times N_a}$ is a quadratic interaction parameter between visible units, where $(i'a',ia)$ element means interaction between $a'$-th sufficient statistics of unit $i'$ at time $t-\delta$ and $a$-th sufficient statistics of unit $i$ at time $t$. \note{check: $\bfW_{j,i}^{[\delta]} = (\bfW_{i,j}^{[\delta]})^\top$??}

\begin{comment}
\item For every $\delta \in [1,\tau]$, $\bfW^{[\delta]}$ has $(N_x + N_h) \times (N_x + N_h)$ elements, and is symmetric
\begin{align} 
\bfW^{[\delta]} =
\begin{bmatrix} 
\bfW_{i,i'}^{[\delta]} & \bfW_{i,j}^{[\delta]} \\
\bfW_{j,i}^{[\delta]} & \bfW_{j,j'}^{[\delta]}
\end{bmatrix},
\end{align}
where $\bfW_{i,i'}^{[\delta]}$ is $N_a \times N_a$ matrix, $\bfW_{i,j}^{[\delta]}$ is $N_a \times N_b$ matrix, $\bfW_{j,j'}^{[\delta]}$ is $N_b \times N_b$ matrix. $\bfW_{i,i'}^{[\delta]} = [w_{ia,i'a'}^{[\delta]}]_{N_a \times N_a}$ is a quadratic interaction parameter between visible units, where $(ia,i'a')$ element means interaction between $a$-th sufficient statistics of unit $i$ at time $t-\delta$ and $a'$-th sufficient statistics of unit $i'$ at time $t$. 
\end{comment}

\smallskip
\item $\Theta = \{ \bmtheta, \bmlambda, \bfU, \bfW^{[\delta]} \}$: model parameters

\smallskip
\item We have a set of of basis functions $\bfV^{[\delta]} = \{ \bfV_{VV}^{[\delta]}, \bfV_{HV}^{[\delta]}, \bfV_{VH}^{[\delta]}, \bfV_{HH}^{[\delta]} \}$. Simply, for weights $\bfW_{i',i}^{[\delta]}$, we define for every $\delta \in [1,\tau]$, for every $i',i = 1, \cdots, N_x$, 
\begin{align}
\bfW_{i',i}^{[\delta]} = \sum_{k=1}^{K_{VV}} \bfA_{i',i,k} \circ \bfV_{VV,k}^{[\delta]}, &\quad \bfW_{j',i}^{[\delta]} = \sum_{k=1}^{K_{HV}} \bfA_{j',i,k} \circ \bfV_{HV,k}^{[\delta]}, \cr 
\bfW_{i',j}^{[\delta]} = \sum_{k=1}^{K_{VH}} \bfA_{i',j,k} \circ \bfV_{VH,k}^{[\delta]}, &\quad \bfW_{j',j}^{[\delta]} = \sum_{k=1}^{K_{HH}} \bfA_{j',j,k} \circ \bfV_{HH,k}^{[\delta]},
\end{align}
where (i) $\bfV_{VV}^{[\delta]}:=[\bfV_{VV,1}^{[\delta]}, \cdots, \bfV_{VV,K_{VV}}^{[\delta]}]$ is the fixed basis matrices (each $\bfV_{VV,k}^{[\delta]}$ is $N_a \times N_a$ basis matrix), (ii) $\bfA_{i',i} := [\bfA_{i',i,1},\cdots,\bfA_{i',i',K_{VV}}]$ are learnable weight matrices for the kernels $\bfW_{i',i}$ (each $\bfA_{i',i,k}$ is $N_a \times N_a$ weight matrix), and (iii) $\mathbf{A} \circ \mathbf{B}$ is the element-wise product of matrix $\mathbf{A}$ and $\mathbf{B}$, known as {\em Hadamard product}, \ie, $(\mathbf{A} \circ \mathbf{B})_{i,j} = (\mathbf{A})_{i,j} (\mathbf{B})_{i,j}$. Then, for a given basis functions $\bfV^{[\delta]}$, we need to learn weights $\bfA = \{ \bfA_{i',i}, \bfA_{j',i}, \bfA_{i',j}, \bfA_{j',j} \}$ (which is regardless of $\delta$). We also defines basis functions for $\bfW_{i,j}, \bfW_{j,i} \bfW_{j',j}, \bfU_{i,j}$ in similar way. $\bfU_{i,j}$ can be assigned as $\bfW_{i,j}^{[0]}$ or $(\bfW_{j,i}^{[0]})^\top$. \note{Connection between basis functions and STDP rule?}

\smallskip
\item Simple case 1: without hidden units. 
We have following form of joint distribution:
\begin{align}
p(\bfx_t | \bfx^{t-1}) \propto \exp \Big\{ \sum_{i} \bmtheta_i^\top \bfs_{i,t} + \sum_{\delta = 0}^\tau \sum_{j,i} \bfs_{j,t-\delta}^\top \bfW_{j,i}^{[\delta]} \bfs_{i,t} \Big\}.
\end{align}
With basis functions, it becomes 
\begin{align} \label{eq:memory-EFH-visible-basis}
p(\bfx_t | \bfx^{t-1}) \propto \exp \Big\{ \sum_{i} \bmtheta_i^\top \bfs_{i,t} + \sum_{\delta = 0}^\tau \sum_{j,i} \bfs_{j,t-\delta}^\top \Big( \sum_{k=1}^K \bfA_{j,i,k} \circ \bfV_k^{[\delta]} \Big) \bfs_{i,t} \Big\},
\end{align}
where $\bfA_{j,i} = \{\bfA_{j,i,1}, \cdots, \bfA_{j,i,K}\}$ are $K$ number of learnable parameter matrices with size $N_a \times N_a$, and $\bfV^{[\delta]} = \{ \bfV_{1}^{[\delta]}, \cdots, \bfV_K^{[\delta]} \}$ is basis functions (matrices) with size $N_a \times N_a$. Then, the model parameters are $\{  \{\bmtheta_i\}_{i=1, \cdots, N_x}, \{ \bfA_{j,i}\}_{i,j = 1, \cdots, N_x} \}$. 

\smallskip
\item Simple case 2: Memoryless visible + Memory hidden units. 
Note that when hidden = visible, this corresponds to the Simple case 1 in \eqref{eq:memory-EFH-visible-basis}.
\begin{align}
p(\bfx_t, \bfh_t | \bfh^{t-1}) ....
\end{align}

\vspace{2cm}
\begin{comment}
\item $\bmth_i := [\theta_{ia}]_{a}, \bml_j := [\lambda_{jb}]_{b}$: singleton parameter of visible unit $i$ and hidden unit $j$. Simply, $\bmth = [\bmth_i]_{i = 1, \cdots, N_x}$ and $\bml = [\bml_j]_{j = 1, \cdots, N_h}$.
\item $\bfW^{[\delta]} := [\bfw_{i',i}^{[\delta]}]_{i',i}$, 
$\bfV^{[\delta]} := [\bfv_{j',i}^{[\delta]}]_{j',i}$, 
$\bfU^{[\delta]} := [\bfu_{i',j}^{[\delta]}]_{i',j}$, 
$\bfZ^{[\delta]} := [\bfz_{j',j}^{[\delta]}]_{j',j}$: quadratic interaction parameter between units with $\delta$ amount of time difference.
\item $\bfw_{i',i}^{[\delta]} := [w_{i'a',ia}^{[\delta]}]_{a',a}$: is a quadratic interaction parameter between visible value of unit $i'$ at time $t-\delta$ and visible value of unit $i$ at time $t$ for each pair of sufficient statistics. $v_{j'b',ia}^{[\delta]}, u_{i'a',jb}^{[\delta]}, z_{j'b',jb}^{[\delta]}$ are defined analogously.
\item $\bfS := [\bfs_{i,j}]_{i,j}$ where $\bfs_{i,j} := [s_{ia,jb}]_{a,b}$ is a quadratic {\em instantaneous} interaction parameter between visible and hidden units for each pair of sufficient statistics. 
\item $\Theta = \{ \bmth,\bml,\bfS,\bfW^{[\delta]},\bfV^{[\delta]},\bfU^{[\delta]},\bfZ^{[\delta]} \}$: model parameters
\end{comment}
\end{enumerate}

\begin{comment}
\smallskip
$\circ$ Joint probability distribution.

\begin{align}
p(\bfx_t,\bfh_t | \bfx^{t-1},\bfh^{t-1}) \propto \exp \bigg[ 
& \sum_{i} \bmth_i^\top \bfs_i(x_{i,t}) + \sum_{j} \bml_j^\top \bfz_j(h_{j,t}) + \sum_{i,j} \bfs_i(x_{i,t})^\top \bfU_{i,j} \bfz_j(h_{j,t}) \cr 
& + \sum_{\delta=1}^\tau \Big[ [\bfs_i(x_{i,t-\delta})^\top]_{i=1,\cdots,N_x}, [\bfh_j(h_{j,t-\delta})^\top]_{j=1,\cdots,N_h} \Big] \bfW^{[\delta]} \cr 
& \qquad \qquad \Big[ [\bfs_i(x_{i,t-\delta})^\top]_{i=1,\cdots,N_x}, [\bfh_j(h_{j,t-\delta})^\top]_{j=1,\cdots,N_h} \Big]^\top
\bigg]
\end{align}

\vspace{0.5cm}

\begin{align} \label{eq:EFH-joint}
p(\bfx_t, \bfh_t | \bfx_{<t}, \bfh_{<t}) \propto 
\exp \bigg[ 
& \sum_{ia} \theta_{ia}f_{ia}(x_{i,t}) + 
\sum_{jb} \lambda_{jb}g_{jb}(h_{j,t}) + 
\sum_{ia,jb} s_{ia,jb}f_{ia}(x_{i,t})g_{jb}(h_{j,t}) \cr 
& +\sum_{\delta=1}^\tau \bigg\{
\sum_{i'a',ia} w_{i'a',ia}^{[\delta]} f_{i'a'}(x_{i',t-\delta}) f_{ia}(x_{i,t}) +
\sum_{j'b',ia} v_{j'b',ia}^{[\delta]} g_{j'b'}(h_{j',t-\delta}) f_{ia}(x_{i,t}) \cr 
& \qquad \qquad + \sum_{i'a',jb} u_{i'a',jb}^{[\delta]} f_{i'a'}(x_{i',t-\delta}) g_{jb}(h_{j,t-\delta}) +
\sum_{j'b',jb} z_{j'b',jb}^{[\delta]} g_{j'b'}(h_{j',t-\delta}) g_{jb}(h_{j,t}) \bigg\} \bigg].
\end{align}
Simply, we consider energy function to represent the probability distribution as $p(\bfx_t, \bfh_t | \bfx_{<t}, \bfh_{<t}) \propto \exp (-E_\Theta(\bfx_t, \bfh_t | \bfx_{<t}, \bfh_{<t}))$, where
\begin{align}
- E_\Theta(\bfx_t, \bfh_t | \bfx_{<t}, \bfh_{<t}) := & \sum_{ia} \theta_{ia}f_{ia}(x_{i,t}) + 
\sum_{jb} \lambda_{jb}g_{jb}(h_{j,t}) + 
\sum_{ia,jb} s_{ia,jb}f_{ia}(x_{i,t})g_{jb}(h_{j,t}) \cr 
& +\sum_{\delta=1}^\tau \bigg\{
\sum_{i'a',ia} w_{i'a',ia}^{[\delta]} f_{i'a'}(x_{i',t-\delta}) f_{ia}(x_{i,t}) +
\sum_{j'b',ia} v_{j'b',ia}^{[\delta]} g_{j'b'}(h_{j',t-\delta}) f_{ia}(x_{i,t}) \cr 
& \qquad \qquad + \sum_{i'a',jb} u_{i'a',jb}^{[\delta]} f_{i'a'}(x_{i',t-\delta}) g_{jb}(h_{j,t-\delta}) +
\sum_{j'b',jb} z_{j'b',jb}^{[\delta]} g_{j'b'}(h_{j',t-\delta}) g_{jb}(h_{j,t}) \bigg\}
\end{align}
\end{comment}

\vspace{2cm}

\smallskip 
$\circ$ Log-likelihood of time-series data for simple case in \eqref{eq:memory-EFH-visible-basis}.

Log-likelihood of time-series data is given by
\begin{align*}
\log p(\bfx^t) = \sum_{s=0}^t \log p(\bfx_s | \bfx^{s-1}),
\end{align*}
thus our goal is to update parameters which maximizes $\log p(\bfx_t | \bfx^{t-1})$ at every step $t$. For each parameter, the gradient of the log-likelihood (element-wise) is  
\begin{align}
\grad_{\bmtheta_i} \log p(\bfx_t | \bfx^{t-1}) &= \mathbb{E}_{\text{data}}\Big[\bfs_{i,t}\Big] - \mathbb{E}_{\text{model}}\Big[\bfs_{i,t}\Big], \cr
\grad_{\bfA_{j,i,k}} \log p(\bfx_t | \bfx^{t-1}) &= \mathbb{E}_{\text{data}}\Big[ \sum_{\delta=0}^\tau \big( \bfs_{j,t-\delta} \bfs_{i,t} \big) \circ \bfV_k^{[\delta]} \Big] - \mathbb{E}_{\text{model}}\Big[ \sum_{\delta=0}^\tau \big( \bfs_{j,t-\delta} \bfs_{i,t} \big) \circ \bfV_k^{[\delta]} \Big],
\end{align}
where data distribution is obtained from the given time-series data $p(\bfx_t | \bfx^{t-1})$, and model distribution is given by \eqref{eq:memory-EFH-visible-basis}. Also, $\bfs_{j, t-\delta} \bfs_{i,t}$ is $N_a \times N_a$ matrix and $\bfV_k^{[\delta]}$ is externally given basis functions. In particular, the gradient with respect to the $(a',a)$-th element of the parameter $\bfA_{j,i,k}$ is obtained by $\sum_{\delta=0}^\tau s_{j,a'}(x_{j,t-\delta}) s_{i,a}(x_{i,t}) \bfV_{k,(a',a)}^{[\delta]}$. 


\vspace{1cm}
\smallskip
$\circ$ Conditional probability distribution. 

% For visible units, 
% \begin{align}
% -E(\bfx_t | \bfx^{t-1}, \bfh^{t}) = \sum_i 
% \end{align}


% \vspace{1cm}
For visible units, 
\begin{align}
-E(\bfx_t | \bfx^{t-1}, \bfh^t) = \sum_{i} \bigg[ \bmtheta_i^\top + \sum_{j} \bfz_{j,t}^\top \bfU_{i,j}^\top + \sum_{\delta=1}^\tau \Big( \sum_{i'} \bfs_{i',t-\delta}^\top \bfW_{i',i}^{[\delta]} + \sum_{j'} \bfz_{j',t-\delta}^\top \bfW_{j',i}^{[\delta]} \Big) \bigg] \bfs_{i,t}.
\end{align}
Note that i) each visible unit $i$ is conditional independent given history (visible + hidden) and current hidden, and ii) this corresponds to a generalized linear model (GLM) if it has linear sufficient statistics $\bfs_i$.

For hidden units, 
\begin{align}
-E(\bfh_t | \bfx^t, \bfh^{t-1}) = \sum_j \bigg[ \bmlambda_j^\top + \sum_{i} \bfs_{i,t}^\top \bfU_{i,j} + \sum_{\delta=1}^\tau \Big( \sum_{i'} \bfs_{i',t-\delta}^\top \bfW_{i',j}^{[\delta]} + \sum_{j'} \bfz_{j',t-\delta}^\top \bfW_{j',j}^{[\delta]} \Big) \bigg] \bfz_{j,t}
\end{align}
Note that i) each hidden unit $j$ is conditional independent given history (visible + hidden) and current visible, and ii) this corresponds to GLM if it has linear sufficient statistics $\bfz_j$.


\note{here..}

\smallskip
$\circ$ Log-likelihood of time-series data.

A goal of learning time-series is to maximize the log-likelihood of a given time-series $\bfx^{t}$. Note that 
\begin{align}
p(\bfx^{t}, \bfh^{t}) = \prod_{s=0}^t p(\bfx_s, \bfh_s | \bfx^{s-1}, \bfh^{s-1}).
\end{align}

Then, the log-likelihood of a given $\bfx^{t}$ is given by
\begin{align} \label{eq:log-likelihood}
\log p(\bfx^{t}) & = \log \sum_{\bfh^{t}} p(\bfx^{t}, \bfh^{t}) \note{check from here..} \cr
& \geq \sum_{\bfh^{t}} \log p(\bfx^{t}, \bfh^{t}) \cr 
& = \sum_{\bfh^{t}} \sum_{s=0}^t \log p(\bfx_s, \bfh_s | \bfx^{s-1}, \bfh^{s-1}) \cr 
& = \sum_{s=0}^t \sum_{\bfh^{s}} \log p(\bfx_s, \bfh_s | \bfx^{s-1}, \bfh^{s-1}) \cr 
& = \sum_{s=0}^t \sum_{\bfh^{s-1}} \sum_{\bfh_s} p(\bfh_s | \bfx^{s}, \bfh^{s-1}) \log p(\bfx_s, \bfh_s | \bfx^{s-1}, \bfh^{s-1}),
\end{align}
where the first inequality holds from Jensen's inequality and the last equality holds for exponential family harmoniums (need to check).

Now, simple algebra gives us the gradient of the log-likelihood in \eqref{eq:log-likelihood} as follows:
\begin{align}
\grad_{\Theta} \log p(\bfx^{t}) = \sum_{s=0}^t \sum_{\bfh^{s-1}} \bigg( \mathbb{E}_{\text{data}}\Big[ - \grad_{\Theta} E_{\Theta}\Big(\bfx_s, \bfh_s | \bfx^{s-1}, \bfh^{s-1}\Big) \Big] - \mathbb{E}_{\text{model}}\Big[ - \grad_{\Theta} E_{\Theta}\Big(\bfx_s, \bfh_s | \bfx^{s-1}, \bfh^{s-1}\Big) \Big]  \bigg).
\end{align}
Here, $\mathbb{E}_{\text{data}}$ is the expectation with respective to the empirical distribution of time-series and $\mathbb{E}_{\text{model}}$ is the expectation with respective to the model distribution in \eqref{eq:EFH-joint}, i.e.,  
\begin{align}
\mathbb{E}_{\text{data}}\left[ \cdot \right] = \sum_{\bfh_s} p(\bfh_s | \bfx^{s}, \bfh^{s-1}) p(\bfx^{s})[\cdot], \quad \mathbb{E}_{\text{model}}\left[ \cdot \right] = \sum_{\bfx_{s}, \bfh_s} p(\bfx_s, \bfh_s | \bfx^{s-1}, \bfh^{s-1})[\cdot].
\end{align}

The gradient for each parameter in \eqref{eq:param-stdp} is now obtained as follows.
\begin{align}
-\grad_{\theta_{ia}} E_{\Theta}(\bfx_s,\bfh_s | \bfx^{s-1},\bfh^{s-1}) & = f_{ia}(x_{i,s}) \cr 
-\grad_{w_{ia,i'a'}^{(P)}} E_{\Theta}(\bfx_s,\bfh_s | \bfx^{s-1},\bfh^{s-1}) & = ...
\end{align}

\vspace{0.5cm}
We can computation of the expectations with the samples drawn from proper distribution. For data distribution, we clamp given time-series data for visible units and obtain samples of hidden units by sampling, and for model distribution, we freely run sampling to obtain samples of visible and hidden units. Need to connect how we can apply {\em contrastive divergence} method in this case.

\vspace{1cm}

\smallskip
$\circ$ Connection to STDP rule: How to define the parameters.

To connect the learning rule with the characteristics of STDP with LTP and LTD, we assume the parameter indicating the interaction between two units of the form in \cite{osogami17:BMtime}. For $\delta \geq 0$, we define the weight as the sum of two weights:
\begin{align}
w_{ia,i'a'}^{[\delta]} = \hat{w}_{ia,i'a'}^{[\delta]} + \hat{w}_{i'a',ia}^{[-\delta]}, 
\end{align}
where 
\begin{align}
\hat{w}_{ia,i'a'}^{[\delta]} = w_{ia,i'a'}^{(P)} \cdot \nu^{\delta-d} \quad ~\text{if}~ \delta \geq d, \quad - w_{ia,i'a'}^{(D)} \cdot \mu^{-\delta}, \quad ~\text{otherwise},
\end{align}
for decay rate $\nu, \mu \in [0,1)$ and delay between pre- and postsynaptic units $d$. We also define other weights $v_{jb,ia}^{[\delta]}, u_{ia,jb}^{[\delta]}, z_{jb,j'b'}^{[\delta]}$ in similar way. In this setting, we note following two points. First, the plasticity between unit $x_i$ and $h_j$ with time difference $\delta$ should be defined in that $\hat{v}_{ia,jb}^{[\delta]} = \hat{u}_{ia,jb}^{[\delta]}$ and $\hat{u}_{jb,ia}^{[\delta]} = \hat{v}_{jb,ia}^{[\delta]}$. Second, it naturally leads to the characterization of the instantaneous correlations between $x_i$ and $h_j$ as
\begin{align}
s_{ia,jb} & = u_{ia,jb}^{[0]} = \hat{u}_{ia,jb}^{[0]}+\hat{u}_{jb,ia}^{[0]} \cr 
& = v_{jb,ia}^{[0]} = \hat{v}_{jb,ia}^{[0]}+\hat{v}_{ia,jb}^{[0]}.
\end{align}
Then, model parameter $\Theta = \{ \bmtheta,\bmlambda,\bfS,\bfW^{[\delta]},\bfV^{[\delta]},\bfU^{[\delta]},\bfZ^{[\delta]} \}$ is equivalent to 
\begin{align} \label{eq:param-stdp}
\{ \bmtheta, \bmlambda, [w_{ia,i'a'}^{(P)}, w_{ia,i'a'}^{(D)}]_{ia,i'a'}, [v_{j'b',ia}^{(P)}, v_{j'b',ia}^{(D)}]_{j'b',ia}, [u_{i'a',jb}^{(P)}, u_{i'a',jb}^{(D)}]_{i'a',jb}, [z_{jb,j'b'}^{(P)}, z_{jb,j'b'}^{(D)}]_{jb,j'b'} \}
\end{align}
for a given $\nu, \mu \in [0,1)$.

\newpage
\noindent {\bf Boltzmann Machine for Time-Series with instantaneous correlations}

Let us now consider this form of undirected models: the probability of spike vector $\mathbf{x}_t$ at time $t$ for a given spike vector trains $\mathbf{x}^{t-1}$ up to time $t-1$,
\begin{align} \label{eq:gbm}
p(\mathbf{x}_t | \mathbf{x}^{t-1}) \propto \exp \bigg( {\bm \gamma}^\top \mathbf{x}_t + \sum_{f=0}^{\tau} \mathbf{x}_{t-f}^\top \mathbf{W}_f \mathbf{x}_t \bigg),
\end{align}
where 
\begin{align}
\mathbf{W}_0 = [w_{0,ij}] = 
\begin{pmatrix}
0 & & & & \\
 & 0 & & & \\
 & & \ddots & & \\
 & & & 0 & \\
 & & & & 0
\end{pmatrix}.
\end{align}

Then, simple algebra provides the following firing probability of neuron $i$ at time $t$ for given history of spike trains $\mathbf{x}^{t-1}$ and other neurons spike status at present $x_{-i,t}$:
\begin{align}
p(x_{i,t} = 1 | x_{-i,t}, \mathbf{x}^{t-1}) = \sigma \Big( \gamma_i + \sum_{f=1}^\tau w_{f,ii} x_{i,t-f} + \sum_{f=0}^\tau \sum_{j \neq i} w_{f,ji} x_{j,t-f} \Big),
\end{align}
where the second term in the sigma function is {\em feedback} kernel and the last term in the sigma function is {\em post-synaptic} kernel of neuron $i$.

Also, in this model, the membrane potential of neuron $i$ at time $t$ is given by
\begin{align}
u_i(t) = \gamma_i + \sum_{f=1}^\tau w_{f,ii} x_{i,t-f} + \sum_{f=0}^\tau \sum_{j \neq i} w_{f,ji} x_{j,t-f}
\end{align}


\vspace{1cm}

\newpage
\underline{\bf We should list up some special cases in existing papers.}

\smallskip
$\circ$ If $\tau = 0$, we obtain a {\em memoryless} Boltzmann Machine with following form:
\begin{align} \label{eq:memorylessbm}
p(\mathbf{x}_t | \mathbf{x}^{t-1}) \propto \exp \bigg( {\bm \gamma}^\top \mathbf{x}_t + \mathbf{x}_t^\top \mathbf{W}_0 \mathbf{x}_t \bigg) = \exp \bigg( \sum_{i} \gamma_i x_{i,t} + \sum_{j \neq i} w_{0,ij}x_{i,t}x_{j,t}  \bigg).
\end{align}

That is, $p(\mathbf{x}_t | \mathbf{x}^{t-1}) = p(\mathbf{x}_t)$. When updating parameters towards MLE, it requires to compute expectation of singleton $x_i$ and pairwise $x_i x_j$ over the distribution $p(\mathbf{x}_t)$. When the number of neurons is large, the computation of the expectation is intractable, therefore, some alternatives (or approximations) can be used: (i) Mean-field approximation, \ie, $p(\mathbf{x}_t) = \prod_{i} p(x_{i,t})$ or equivalently $\mathbf{W}_0 = \mathbf{0}$. (ii) Gibbs sampler which draws random samples from the distribution $p(\mathbf{x}_t)$ using local values. (iii) Contrastive Divergence which draws random samples from the contrastive distribution $p_\ell(\mathbf{x}_t)$, via Gibbs sampler at step $\ell$. (iv) GAN-based approach to discriminative the target (data) distribution samples and model distribution samples. 


\vspace{1cm}


\newpage
\smallskip
$\circ$ For $\tau > 0$, we have a {\em memory} Boltzmann Machine. For finite $\tau > 0$, it considers the past of length $\tau$ as DyBM-T does. For $\tau = \infty$, the model takes account of the entire history. 

\vspace{1cm}

\smallskip
$\circ$ Winner-Take-All (WTA) circuit in \cite{kappel15:synaptic,habenschuss13:stdp}

In WTA circuit, only one neuron can fire a spike at present. This model can be represented by setting a weight matrix $\mathbf{W}_0$ as follows: for all $i \neq j$, $w_{0,ij} = - \infty$, \ie, 
\begin{align} \label{eq:wta_matrix}
\mathbf{W}_0 = [w_{0,ij}] = 
\begin{pmatrix}
0 & & & & \\
 & 0 & & -\infty & \\
 & & \ddots & & \\
 & -\infty & & 0 & \\
 & & & & 0
\end{pmatrix}.
\end{align}
Note that this is similar to the {\em hard-core} graphical model, where every adjacent nodes cannot be active simultaneously, since general BM assumes completely connected structure. 

Also note that this WTA model does consider the instantaneous pair-wise correlations between neurons, \ie, considering $\mathbf{W}_0$ as defined in \eqref{eq:wta_matrix}. Most of existing models of SNNs assume the {\em conditional independent} instantaneous firing of neurons in that $\mathbf{W}_0 = \mathbf{0}$. 

Firing probability of neuron $i$ at time $t$ is $\rho_i(t)$:
\begin{align*}
\rho_i(t) = \frac{\exp(u_i(t))}{\sum_{j} \exp(u_j(t))},
\end{align*}
where the membrane potential is 
\begin{align*}
u_i(t) = \gamma_i + \sum_{f=1}^\tau x_{i,t-f} w_{f,ii} + \sum_{j \neq i} \sum_{f=1}^\tau x_{j,t-f} w_{f,ji}.
\end{align*}

Remark that the membrane potential of WTA defined in synaptic sampling paper \cite{kappel15:synaptic} has form of
\begin{align} \label{eq:wtas_potential}
u_i(t) = \beta_i(t) + \sum_{j \neq i} w_{ij} x_j(t),
\end{align} 
where for spiking times of neuron $i$ is $\{ t_i^{(f)} \}$
\begin{align} \label{eq:wtas_kernels}
\beta_i(t) = \gamma \cdot \sum_{f=1}^\tau \kappa(t - t_i^{(f)}), ~ \quad ~ \text{and} ~ \quad ~ x_j(t) = \sum_{f=1}^\tau \epsilon(t - t_j^{(f)}).
\end{align}
Note that $w_{ij}$ in \eqref{eq:wtas_potential} and $\gamma$ in \eqref{eq:wtas_kernels} are different to that of our models \eqref{eq:gbm}. Please clarify the specific matching these two representations with special choice of ${\bm \gamma}, \mathbf{W}_f$ in \eqref{eq:gbm} related to $\gamma, \kappa, \epsilon, w$ in \eqref{eq:wtas_potential} and \eqref{eq:wtas_kernels}. How the spiking times $\{ t_i^{(f)} \}$ of neuron $i$ can be understood in our framework? 

\vspace{1cm}

\newpage 
\smallskip
$\circ$ GLM neurons in \cite{bagheri17:snn_first}.

In Bernoulli Generalized Linear Model (GLM) neuron, the membrane potential of post-synaptic neuron $i$ at time $t$ is given by 
\begin{align} \label{eq:glm_potential}
u_i(t) = \sum_{j \neq i} {\bm \alpha}_{j,i}^\top x_{j}^{[t-\tau: t-1]} + {\bm \beta}_i^\top y_i^{[t-\tau:t-1]} + \gamma_i.
\end{align}
Here, the model explicit causal relationship (fixed post- and presynaptic neurons) and it cares about discriminative model, \ie, considering following probability of spike train of postsynaptic neuron for given spike trains of input neurons $p(y_{i,t}|\mathbf{x}^{t-1}, y_i^{t-1})$.

One single postsynaptic neuron $i$, no instantaneous pair-wise (pre-post) correlations, 

\begin{align} \label{eq:glm}
p(y_{i,t} | \mathbf{x}^{t-1}, y_i^{t-1}) \propto \exp (u_i(t)) &= \exp \bigg( \gamma_i y_{i,t} + {\bm \beta}_i^\top y_i^{[t-\tau:t-1]} +  \sum_{j \neq i} {\bm \alpha}_{j,i}^\top x_{j}^{[t-\tau: t-1]} \bigg) \cr 
& = \exp \bigg( \gamma_i y_{i,t} + \sum_{f=1}^\tau y_{i,t-f} \beta_{f,i} y_{i,t} + \sum_{f=1}^\tau \mathbf{x}_{t-f}^\top {\bm \alpha}_f y_{i,t}  \bigg).
\end{align}

Thus, the firing probability of post-synaptic neuron $i$ at time $t$ is 
\begin{align}
\rho_i(t) = p(y_{i,t}=1 | y_i^{t-1}, \mathbf{x}^{t-1}) = \sigma (u_i(t))
\end{align}

\vspace{1cm}

\newpage 
\smallskip
$\circ$ Spiking Boltzmann Machine in \cite{hinton00:sBM}.

In general Spiking Boltzmann Machine (SBM), it has a single hidden layer and a single visible layer with restricted structure (\ie, no inside-layer connection). 

\begin{align} \label{eq:sbm}
p(\mathbf{x}_t, \mathbf{h}_t | \mathbf{x}^{t-1}, \mathbf{h}^{t-1}) \propto \exp \bigg( & ({\bm b}^V)^\top \mathbf{x}_t + ({\bm b}^H)^\top \mathbf{h}_t + \mathbf{h}_t^\top r(0) \mathbf{W}^{HV} \mathbf{x}_t \cr & + \sum_{f=1}^\infty r(f) \cdot \big( \mathbf{h}_{t-f}^\top \mathbf{W}^{HH} \mathbf{h}_{t} + \mathbf{h}_{t-f}^\top \mathbf{W}^{HV} \mathbf{x}_{t} + \mathbf{x}_{t-f}^\top \mathbf{W}^{VH} \mathbf{h}_{t} + \mathbf{x}_{t-f}^\top \mathbf{W}^{VV} \mathbf{x}_{t} \big) \bigg),
\end{align}

We can obtain followings by comparing \eqref{eq:gbm} and \eqref{eq:sbm}. 

The spiking BM with no hidden layer, \ie, $\mathbf{h}_{(\cdot)} = \emptyset$, it does not include the correlation between visible nodes and visible nodes at present. In other words, it lacks of instantaneous pair-wise correlation: $\mathbf{x}_t - \mathbf{x}_t$ and $\mathbf{h}_t - \mathbf{h}_t$. 

Also, this model reduces the number of parameters of the model by taking an arbitrarily chosen function $r(f)$ for every time $f$. The model parameter of control is: $\mathbf{b}^V, \mathbf{b}^H, \mathbf{W}^{VV}, \mathbf{W}^{VH}, \mathbf{W}^{HV}, \mathbf{W}^{HH}$. 


\vspace{1cm}

\newpage 
\smallskip
$\circ$ Dynamic Boltzmann Machine (DyBM) in \cite{osogami15:DyBM,osogami17:BMtime}.

For a finite $T>0$, we have:
\begin{align} \label{eq:dybm_T}
p(\mathbf{x}_t | \mathbf{x}^{[t-T+1:t-1]}) \propto \exp \bigg( \textbf{b}^\top \mathbf{x}_t + \sum_{f=1}^{T-1} \mathbf{x}_{t-f}^\top \mathbf{W}_f \mathbf{x}_{t} \bigg),
\end{align}

We can obtain followings by comparing \eqref{eq:gbm} and \eqref{eq:dybm_T}. The DyBM is a special case in that it does not include instantaneous pair-wise correlation: $\mathbf{x}_t - \mathbf{x}_t$, thus it considers {\em strict causality}. 

To have a learning rule with the characteristics of STDP with LTP and LTD, the DyBM-T defines the weight $w_{f,ij}$ for $f > 0$ as the sum of two weights, $\hat{w}_{f,ij}$ and $\hat{w}_{f,ji}$: 
\begin{align} \label{eq:dybm_weight}
w_{f,ij} = \hat{w}_{f,ij} + \hat{w}_{f,ji}.
\end{align}
In general, this weight is {\em asymmetric}: $w_{f,ij} \neq w_{f,ji}$ for all $j \neq i$. However, we also observe 
$$w_{f,ij} = w_{-f, ji}.$$
The STDP function $\hat{\mathbf{W}}_{f}$ is parameterized by $\mathbf{U}$ and $\mathbf{V}$, see \cite{osogami17:BMtime,osogami15:DyBM} for detailed shape of the STDP function. The model parameter of control is: $\mathbf{b}, \mathbf{U}, \mathbf{V}$ with hyperparameter $\lambda, \mu$ used to define the STDP function, \ie
\begin{align*}
\hat{w}_{f,ij} = u_{ij} \lambda^{f - d_{ij}} ~~\text{for LTP,} \qquad \hat{w}_{f,ij} = -v_{ij} \mu^{-f} ~~ \text{for LTD}.
\end{align*}

\vspace{1cm}

$\circ$ Dynamic Boltzmann machine (DyBM) with hidden variables: RBM structure.

\begin{align} \label{eq:dyrbm_T}
E_{\theta,\phi}(\mathbf{x}_t, \mathbf{h}_t | \mathbf{x}^{t-1}, \mathbf{h}^{t-1}) = E_{\theta}(\mathbf{x}_t | \mathbf{x}^{t-1}, \mathbf{h}^{t-1}) + E_{\phi}(\mathbf{h}_t | \mathbf{x}^{t-1}, \mathbf{h}^{t-1}),
\end{align}
and the log-likelihood of the visible time-series $\mathbf{x}^t$ and its lower bound is given by:
\begin{align*}
\log p_{\theta,\phi}(\mathbf{x}^t) = \log \Big( \sum_{\mathbf{h}^t} p_{\phi}(\mathbf{h}^t | \mathbf{x}^t) \prod_{s=1}^t p_{\theta}(\mathbf{x}_s | \mathbf{x}^{s-1}, \mathbf{h}^{s-1}) \Big)
\end{align*}


% On 061018
\smallskip
\noindent {\bf Generalized Linear Models (GLM)} in \cite{bagheri17:snn_first}.

\note{need to modify notations.}

In Bernoulli Generalized Linear Model (GLM) neuron, the membrane potential of post-synaptic neuron $i$ at time $t$ is given by 
\begin{align} \label{eq:glm_potential}
u_i(t) = \sum_{j \neq i} {\bm \alpha}_{j,i}^\top x_{j}^{[t-\tau: t-1]} + {\bm \beta}_i^\top y_i^{[t-\tau:t-1]} + \gamma_i.
\end{align}
Here, the model explicit causal relationship (fixed post- and presynaptic neurons) and it cares about discriminative model, \ie, considering following probability of spike train of postsynaptic neuron for given spike trains of input neurons $p(y_{i,t}|\mathbf{x}^{t-1}, y_i^{t-1})$.

One single postsynaptic neuron $i$, no instantaneous pair-wise (pre-post) correlations, 

\begin{align} \label{eq:glm}
p(y_{i,t} | \mathbf{x}^{t-1}, y_i^{t-1}) \propto \exp (u_i(t)) &= \exp \bigg( \gamma_i y_{i,t} + {\bm \beta}_i^\top y_i^{[t-\tau:t-1]} +  \sum_{j \neq i} {\bm \alpha}_{j,i}^\top x_{j}^{[t-\tau: t-1]} \bigg) \cr 
& = \exp \bigg( \gamma_i y_{i,t} + \sum_{f=1}^\tau y_{i,t-f} \beta_{f,i} y_{i,t} + \sum_{f=1}^\tau \mathbf{x}_{t-f}^\top {\bm \alpha}_f y_{i,t}  \bigg).
\end{align}

Thus, the firing probability of post-synaptic neuron $i$ at time $t$ is 
\begin{align}
\rho_i(t) = p(y_{i,t}=1 | y_i^{t-1}, \mathbf{x}^{t-1}) = \sigma (u_i(t))
\end{align}

\vspace{1cm}

\smallskip
\noindent {\bf Boltzmann Machines for Time-series} in \cite{osogami15:DyBM,osogami17:BMtime}.

\note{need to modify notations.}

For a finite $T>0$, we have:
\begin{align} \label{eq:dybm_T}
p(\mathbf{x}_t | \mathbf{x}^{[t-T+1:t-1]}) \propto \exp \bigg( \textbf{b}^\top \mathbf{x}_t + \sum_{f=1}^{T-1} \mathbf{x}_{t-f}^\top \mathbf{W}_f \mathbf{x}_{t} \bigg),
\end{align}

We can obtain followings by comparing our model and \eqref{eq:dybm_T}. The DyBM is a special case in that it does not include instantaneous pair-wise correlation: $\mathbf{x}_t - \mathbf{x}_t$, thus it considers {\em strict causality}. 

To have a learning rule with the characteristics of STDP with LTP and LTD, the DyBM-T defines the weight $w_{f,ij}$ for $f > 0$ as the sum of two weights, $\hat{w}_{f,ij}$ and $\hat{w}_{f,ji}$: 
\begin{align} \label{eq:dybm_weight}
w_{f,ij} = \hat{w}_{f,ij} + \hat{w}_{f,ji}.
\end{align}
In general, this weight is {\em asymmetric}: $w_{f,ij} \neq w_{f,ji}$ for all $j \neq i$. However, we also observe 
$$w_{f,ij} = w_{-f, ji}.$$
The STDP function $\hat{\mathbf{W}}_{f}$ is parameterized by $\mathbf{U}$ and $\mathbf{V}$, see \cite{osogami17:BMtime,osogami15:DyBM} for detailed shape of the STDP function. The model parameter of control is: $\mathbf{b}, \mathbf{U}, \mathbf{V}$ with hyperparameter $\lambda, \mu$ used to define the STDP function, \ie
\begin{align*}
\hat{w}_{f,ij} = u_{ij} \lambda^{f - d_{ij}} ~~\text{for LTP,} \qquad \hat{w}_{f,ij} = -v_{ij} \mu^{-f} ~~ \text{for LTD}.
\end{align*}

\vspace{1cm}

\smallskip
\noindent {\bf Winner-Take-All (WTA) Circuits} in \cite{kappel15:synaptic,habenschuss13:stdp}.

\note{need to modify notations.}

In WTA circuit, only one neuron can fire a spike at present. This model can be represented by setting a weight matrix $\mathbf{W}_0$ as follows: for all $i \neq j$, $w_{0,ij} = - \infty$, \ie, 
\begin{align} \label{eq:wta_matrix}
\mathbf{W}_0 = [w_{0,ij}] = 
\begin{pmatrix}
0 & & & & \\
 & 0 & & -\infty & \\
 & & \ddots & & \\
 & -\infty & & 0 & \\
 & & & & 0
\end{pmatrix}.
\end{align}
Note that this is similar to the {\em hard-core} graphical model, where every adjacent nodes cannot be active simultaneously, since general BM assumes completely connected structure. 

Also note that this WTA model does consider the instantaneous pair-wise correlations between neurons, \ie, considering $\mathbf{W}_0$ as defined in \eqref{eq:wta_matrix}. Most of existing models of SNNs assume the {\em conditional independent} instantaneous firing of neurons in that $\mathbf{W}_0 = \mathbf{0}$. 

Firing probability of neuron $i$ at time $t$ is $\rho_i(t)$:
\begin{align*}
\rho_i(t) = \frac{\exp(u_i(t))}{\sum_{j} \exp(u_j(t))},
\end{align*}
where the membrane potential is 
\begin{align*}
u_i(t) = \gamma_i + \sum_{f=1}^\tau x_{i,t-f} w_{f,ii} + \sum_{j \neq i} \sum_{f=1}^\tau x_{j,t-f} w_{f,ji}.
\end{align*}

Remark that the membrane potential of WTA defined in synaptic sampling paper \cite{kappel15:synaptic} has form of
\begin{align} \label{eq:wtas_potential}
u_i(t) = \beta_i(t) + \sum_{j \neq i} w_{ij} x_j(t),
\end{align} 
where for spiking times of neuron $i$ is $\{ t_i^{(f)} \}$
\begin{align} \label{eq:wtas_kernels}
\beta_i(t) = \gamma \cdot \sum_{f=1}^\tau \kappa(t - t_i^{(f)}), ~ \quad ~ \text{and} ~ \quad ~ x_j(t) = \sum_{f=1}^\tau \epsilon(t - t_j^{(f)}).
\end{align}
Note that $w_{ij}$ in \eqref{eq:wtas_potential} and $\gamma$ in \eqref{eq:wtas_kernels} are different to that of our models. Please clarify the specific matching these two representations with special choice of ${\bm \gamma}, \mathbf{W}_f$ in our models related to $\gamma, \kappa, \epsilon, w$ in \eqref{eq:wtas_potential} and \eqref{eq:wtas_kernels}. How the spiking times $\{ t_i^{(f)} \}$ of neuron $i$ can be understood in our framework? 

\vspace{2cm}


\smallskip
\noindent {\bf Factorization over connected components of the lateral graph.}
In general, the lateral graph $\set{G}_{\set{L}}$ can be decomposed into an $L$ number of disjoint connected components. An $l$-th connected component $\set{C}_l$ is defined as a subset of units in which any two units are connected to each other by paths where a path is a sequence of edges in $\set{E}_{\set{L}}$, and which is connected to no additional units in $\set{V} \setminus \set{C}_l$. We denote by $\set{C}(i)$ the connected component associated with unit $i$, \ie, $\set{C}(i)$ is the set of units (including unit $i$) that are connected to unit $i$. Then, the model \eqref{eq:DEF} is represented in following factorization form over $L$ connected components
\begin{align} \label{eq:DEF-connected}
p(\bmx_t | \bmx^{t-1},\Theta) = \prod_{l=1}^L p(\bmx_{\set{C}_l,t} | \bmx^{t-1}_{\set{P}_{\set{C}_l}},\Theta) = \prod_{l=1}^L p(\bmx_{\set{C}_l,t} | \bmalpha_{\set{P}_{\set{C}_l},t-1},\Theta).
\end{align}

\smallskip
\noindent {\bf Distributed computation of the gradients: Gibbs sampler.}
We now discuss the information required to compute the gradients \eqref{eq:DEF-ll-grad} for each unit $i$. The positive components require the sufficient statistics $\bms_{i,t}$ and the filtered traces $\bmalpha_{j,t-1}$ for all parents $j \in \set{P}_i$ of the node. In contrast, the negative components entail the computation of the average of the relevant sufficient statistics over the {\em marginal} distribution of each unit $i$ or edge $(j,i) \in \set{E}_{\set{P}}, \set{E}_{\set{L}}$. Specifically, in \eqref{eq:DEF-ll-grad-th}, the expectation $\mathbb{E}_{\bfx_t \sim p(\bmx_t|\bmx^{t-1},\Theta)}[\bfs_{i,t}|\bmx^{t-1}]$ is over the marginal distribution $p(x_{i,t} | \bmx^{t-1},\Theta)$, which is given as
\begin{align}
p(x_{i,t}|\bmx^{t-1},\Theta) %= \sum_{\bmx_{\set{V} \setminus \{i\},t}} p(\bmx_t|\bmx^{t-1},\Theta) 
= \sum_{\bmx_{\mathtt{cn}_i,t}} p(x_{i,t}, \bmx_{\mathtt{cn}_i,t} | \bmalpha_{\set{P}_{\set{C}_i}, t-1}, \Theta),
\end{align}
where we recall that $\set{C}_i = \mathtt{cn}_i \cup \{i\}$ is the set of units that are reached to unit $i$ via lateral connections, see Appendix for details. In practice, the average in \eqref{eq:DEF-ll-grad-th} can hence be computed ... \note{Gibbs sampling....} 
\begin{align*}
\mathbb{E}_{\bfx_t \sim p(\bmx_t|\bmx^{t-1},\Theta)}[\bfs_{i,t}|\bmx^{t-1}] &= \mathbb{E}_{\rmx_{i,t} \sim p_i(x_{i,t}|\bmalpha_{\set{P}_{\{i\} \cup \set{C}_i}},\Theta)} \big[ \bfs_{i,t} \big] \cr 
&= \sum_{x_{i,t}} p_i(x_{i,t}|\bmx^{t-1},\Theta) \bms_i(x_{i,t}) = \sum_{x_{i,t}} \sum_{\bmx_{\set{C}_i,t}} p(x_{i,t},\bmx_{\set{C}_i,t} | \bmalpha_{\set{P}_{\{i\} \cup \set{C}_i}},\Theta) \bms_i(x_{i,t}),
\end{align*}
which in turn requires knowledge of the filtered traces of units that are causally connected to either the unit $i$ itself or the units that are reached unit $i$ via lateral connections. 
For \eqref{eq:DEF-ll-grad-V}, given filtered trace $\bmalpha_j$ of the unit $j \in \set{P}_i$, the expectation term is computed over the marginal distribution $p_i(x_{i,t} | \bmx^{t-1},\Theta)$ of unit $i$. For \eqref{eq:DEF-ll-grad-U}, the expectation $\mathbb{E}_{\bfx_t \sim p(\bmx_t|\bmx^{t-1},\Theta)}[\bfs_{j,t}\bfs_{i,t}^\top|\bmx^{t-1}]$ is computed over the marginal distribution $p(x_{j,t}x_{i,t} | \bmx^{t-1},\Theta)$, given as
\begin{align}
p(x_{j,t},x_{i,t}|\bmx^{t-1},\Theta) %= \sum_{\bmx_{\set{V} \setminus \{i,j\},t}} p(\bmx_t|\bmx^{t-1},\Theta) 
= \sum_{\bmx_{\mathtt{Cn}_j \cup \mathtt{Cn}_i,t}} p(x_{j,t},x_{i,t}, \bmx_{\mathtt{Cn}_j \cup \mathtt{Cn}_i,t} | \bmalpha_{\set{P}_{\set{C}(i) \cup \set{C}(j)},t-1}, \Theta),
\end{align}
thus in turn requires knowledge of the filtered traces of units that are causally connected to either the unit $i$ or unit $j$ or all units that are reached to $i$ or $j$ via lateral connections.

As a spiking neural network, the SNN has $N_x$ number of neurons and $\bfx_t = (\rmx_{1,t},\cdots,\rmx_{N_x,t})$ is the spiking behaviors of the neurons at time $t=1,2,\cdots$, where $\rmx_{i,t}$ is the binary signal, or spike, emitted by neuron $i$ at time $t$. Also, we let $\bfx_i^t=(\rmx_{i,1},\cdots, \rmx_{i,t})$ be the spike train of neuron $i$ from time $1$ to $t$, and the sequence of random process $\bfx^t = (\bfx_1,\cdots,\bfx_t)$ is the entire spike trains of neurons from time $1$ to $t$. Accordingly, the joint distribution of the entire spike trains is given by the factorized form in \eqref{eq:DEF-joint-time}, with a set of model parameters $\Theta$. We note that each neuron $i$ has one-dimensional sufficient statistic $s_i(x_i) = x_i$ and natural parameter $\theta_i$, or the bias parameter of the neuron.  

\noindent {\bf SNN with GLM neurons.} 
The spiking behavior of each neuron at each time $t$ is Bernoulli distributed \cite{bagheri17:snn_first}, then the firing probability of neurons can be represented as \eqref{eq:DEF} or \eqref{eq:DEF-filtered} with following coincidence: 
%{\em (i)} each neuron $i$ has one-dimensional sufficient statistic $s_i(x_i) = x_i$ and natural parameter $\theta_i$, or the bias parameter of the neuron, {\em (ii)} 
{\em (i)} this model has no consideration of instantaneous correlations among neurons, \ie, all-zero matrices $\bfU$, {\em (ii)} the term $\sum_{k=1}^K \bfV_{i,i,k}^\top \bmalpha_{i,k,t-1}$ corresponds to the {\em feedback kernel} of neuron $i$, and {\em (iii)} the term $\sum_{k=1}^K \bfV_{j,i,k}^\top \bmalpha_{j,k,t-1}$ corresponds to the {\em synaptic kernel} applied on the synapse between neuron $j \in \set{P}_i$ and $i$. We note that the firing probability depends on the past spiking behaviors in a window of duration $\tau$ samples. 


%% gibbs sampler
\note{Here...} In contrast, the negative components entail the computation of the average of the relevant sufficient statistics over the model distribution, which in practice can be computed by using the {\em Gibbs sampler} in following way. The Gibbs sampler for $p(\bmx_t | \bmx^{t-1},\Theta)$ generates a sequence of $M$ draws, where we denote by $\bfx_{t}^{(m)}$ the $m$-th sample. We begin with some initial value $\bfx_{t}^{(0)}$ and at iteration $m$, the value $\rmx_{i,t}^{(m)}$ of unit $i$ is drawn based on the following conditional distribution 
\begin{align}
p(x_{i,t} | \bmx_{\set{V} \setminus \{i\}, t}, \bmx^{t-1},\Theta) &= p(x_{i,t} | \bmx_{\set{L}_i,t}, \bmalpha_{\set{P}_i,t-1}, \Theta) \cr 
&\propto \exp \Big\{ \big( \bmtheta_i + \sum_{j \in \set{P}_i} \sum_{k=1}^K \bfV_{j,i,k}^\top \bmalpha_{j,k,t-1} \big)^\top \bms_{i,t} + \sum_{j \in \set{L}_i} \bms_{j,t}^\top \bfU_{j,i} \bms_{i,t}  \Big\} \cr 
&:= \exp \big\{ \bmr_{i,t}^\top \bms_{i,t} \big\},
\end{align}
where we define the conditioned energy, or a membrane potential, $\bmr_{i,t}$ of unit $i$ at time $t$ as
\begin{align}
\bmr_{i,t} = \bmtheta_i + \sum_{j \in \set{P}_i} \sum_{k=1}^K \bfV_{j,i,k}^\top \bmalpha_{j,k,t-1} + \sum_{j \in \set{L}_i} \bfU_{j,i}^\top \bms_{j,t}.
\end{align}
This process is repeated until obtaining $M$ samples, then the negative components are computed by 
%$\frac{1}{M} \sum_{m=1}^M \bms_i(\rmx_{i,t}^{(m)})$ in \eqref{eq:DEF-ll-grad-th}, $\frac{1}{M} \sum_{m=1}^M \bmalpha_{j,t-1} \bms_i(\rmx_{i,t}^{(m)})$ for all $j \in \set{P}_i$ in \eqref{eq:DEF-ll-grad-V}, and finally $\frac{1}{M} \sum_{m=1}^M \bms_j(\rmx_{j,t}^{(m)}) \bms_i(\rmx_{i,t}^{(m)})^\top$ for all $j \in \set{L}_i$ in \eqref{eq:DEF-ll-grad-U}.
\begin{align*}
\frac{1}{M} \sum_{m=1}^M \bms_i(\rmx_{i,t}^{(m)}), \quad \frac{1}{M} \sum_{m=1}^M \bmalpha_{j,t-1} \bms_i(\rmx_{i,t}^{(m)}), \quad \frac{1}{M} \sum_{m=1}^M \bms_j(\rmx_{j,t}^{(m)}) \bms_i(\rmx_{i,t}^{(m)})^\top,
\end{align*}
in \eqref{eq:DEF-ll-grad-th}, \eqref{eq:DEF-ll-grad-V}, and \eqref{eq:DEF-ll-grad-U}, respectively. 


% STDP connection

In this setting, the gradient of the log-likelihood for $\bfV$ is given as: for $k=1,\cdots,M$, 
\begin{align}
\grad_{\rmV_{j,i,2k-1}} \ln p(\bmx_t | \bmx^{t-1},\Theta) 
&= \alpha_{j,2k-1,t-1} \Big( x_{i,t} - \mathbb{E}_{\Theta} \big[ \rmx_{i,t} | \bmx^{t-1} \big] \Big), \cr
%&= \Big( \sum_{\delta=d}^\tau \lambda_{2k-1}^{\delta-d} x_{j,t-\delta} \Big) \Big( x_{i,t} - \mathbb{E}_{\Theta} \big[ \rmx_{i,t} | \bmx^{t-1} \big] \Big), \quad ~\text{for}~ k \in [1,M] \cr
\grad_{\rmV_{j,i,2k}} \ln p(\bmx_t | \bmx^{t-1}, \Theta) &= \alpha_{j,2k,t-1} \Big( -x_{i,t} + \mathbb{E}_{\Theta} \big[ \rmx_{i,t} | \bmx^{t-1} \big] \Big).
%\grad_{\rmV_{j,i,2k}} \ln p(\bmx_t | \bmx^{t-1}, \Theta) &= \big( \sum_{\delta=1}^d \mu_k^{-\delta} \bfs_{j,t-\delta} \big) \Big( -\bfs_{i,t} + \mathbb{E}_{\Theta} \big[ {\bm s}_{i,t} | \bfx^{t-1} \big] \Big)^\top, \quad ~\text{for}~ k \in [M+1,2M].
\end{align}
This learning rule exhibits LTP and LTD properties with STDP in that the amount of the change in the weight between two neurons that fired together depends on the precise timings when the two neurons fired. First, the odd-numbered synaptic weight matrix $\rmV_{j,i,2k-1}$ for $k=1,\cdots,M$, which is associated with LTP-type basis functions \eqref{eq:basis-stdp-ltp}, is increased, \ie, LTP gets stronger, when $x_{i,t}=1$ is given. Then, the neuron $i$ becomes more likely to fire when filtered signal from $j$ have recently and frequently arrived, \ie, $\alpha_{j,2k-1,t-1}$ is large. In contrast, associated with LTD-type basis functions \eqref{eq:basis-stdp-ltd}, the even-numbered synaptic weight matrix $\rmV_{j,i,2k}$ for $k=1,\cdots,M$ is increased, \ie, LTD gets stronger, when $x_{i,t}=0$ is given. Then, the neuron $i$ becomes less likely to fire when filtered signal from $j$ are expected to reach $i$ soon, \ie, $\alpha_{j,2k,t-1}$ is large. 

For convenience, we denote the filtered signal associated with two types of basis functions as positive quantities by
\begin{align}
\alpha_{j,2k-1,t} = \sum_{\delta=0}^{\tau-1} \lambda_{2k-1}^{[\delta+1-d]} \cdot 1_{\{\delta+1 \geq d\}} \cdot x_{j,t-\delta}, \quad \alpha_{j,2k,t} = \sum_{\delta=0}^{\tau-1} \lambda_{2k}^{[-\delta-1]} \cdot 1_{\{ \delta+1 < d \}} \cdot x_{j,t-\delta},
\end{align}
for $k=1,\cdots,M$; and denote the membrane potential $r_{i,t}$ of neuron $i$ at time $t$ by 
\begin{align*}
r_{i,t} = \theta_i + \sum_{j \in \set{P}_i} \Big( \sum_{k=1}^M \alpha_{j,2k-1,t-1} v_{j,i,2k-1} - \alpha_{j,2k,t-1} v_{j,i,2k} \Big).
\end{align*}
Then, the gradient of the log-likelihood for $\bfV$ is given as 
\begin{align}
\grad_{v_{j,i,2k-1}} \ln p(\bmx_t | \bmx^{t-1},\Theta) &= \alpha_{j,2k-1,t-1} \big( x_{i,t} - g(r_{i,t}) \big) \cr
\grad_{v_{j,i,2k}} \ln p(\bmx_t | \bmx^{t-1},\Theta) &= \alpha_{j,2k,t-1} \big( -x_{i,t} + g(r_{i,t}) \big),
\end{align}


%% Numerical results
First, the goal is to evaluate whether, when a set of time-series data is generated from our dynamic exponential family model, the learning methods in Section~\ref{sec:learning} can learn the underlying model from a given set of time-series data. To this end, we first set a dynamic exponential family model: a causal graph $\set{G}_{\set{P}}$ is a complete graph; a lateral graph consists of two WTA circuits, \ie, each half of the neurons are fully connected with each other, and these two groups are disjoint; the $K$ basis functions $a_k$ are either raised cosine functions or STDP functions; a memory parameter $\tau > 0$; we have a following model parameter $\Theta_{\text{true}} = \{ \bmtheta, \bfV, \bfU \}$ - $\theta_i$ for $i \in \set{V}$ are randomly chosen, $v_{j,i,k}$ for $(j,i) \in \set{V}^2$ and $k = 1,\cdots,K$ are randomly chosen, and $u_{j,i}$ for $(j,i) \in \set{V}^2$ is set as (not exact... briefly) 
\begin{align}
\bfU = 
\begin{bmatrix}
-\infty & {\bm 0} \\
{\bm 0} & -\infty
\end{bmatrix}
\end{align}
Then, we generate time-series data $\bmx_t$ for $t=1,\cdots,$ from the conditional joint distribution \eqref{eq:DEF-basis}. We then train the model from data using either ML learning algorithm described in Section~\ref{sec:mle-learning} or Langevin algorithm described in Section~\ref{sec:langevin-learning}. 

\noindent (NOTE: How to evaluate the performance??) One possible way is a prediction. From the trained model, we predict the $p(\bmx_{T+1}|\bmx^T, \Theta)$ for a given test data $\bmx^T$, and evaluate the performance, \eg, cross entropy with $p(\bmx_{T+1}| \bmx^T, \Theta_{\text{true}})$.

Next, we can have classification for MNIST dataset with a two-layer SNN. We consider two class of digits $\{1,7\}$. The neurons $\set{V}$ consists of two layers: the first layer is input neurons, \ie, each pixel of digit image corresponds to each neuron in input layer; the second layer is output neurons, \ie, two output neurons correspond to a label of the digit image, $1$ or $7$, and two output neurons correspond to an orientation of the digit image, vertical or horizontal. This two-layer SNN can be represented as a dynamic exponential family. First, there are causal connections only from input neurons to output neurons. No self-loop connection is considered. Second, there are lateral connections only between label-type output neurons, and only between orientation-type output neurons. 

\noindent (NOTE: need to clarify in detail for spike trains generations, encoding/decoding.) A digit image (with a label and orientation) can be converted to input/output spike trains by generating i.i.d. Bernoulli vectors (or Poisson-distributed), using rate encoding/decoding. From a given dataset, we train the model starting from a random initial model parameter, and evaluate the classification accuracy in terms of label. 


\begin{figure}[t]
  \centering
   \includegraphics[width=0.47\columnwidth]{fig/information_gradient}
  \caption{The information required to compute the gradients \eqref{eq:DEF-ll-grad} for each unit $i$. For positive component in \eqref{eq:DEF-ll-grad-U}, the current sufficient statistics $\bfs_{j,t}$ for all units $j \in \set{L}_i$ connected by a lateral link are required. For positive component in \eqref{eq:DEF-ll-grad-V} and/or the negative components in \eqref{eq:DEF-ll-grad}, the local filtered traces $\bmalpha_{j',t-1}$ for all units $j' \in \set{P}_{\set{C}_i \cup \{i\}}$ reachable to unit $i$ via causal and lateral links are required.}
  \label{fig:grad_info}
\end{figure}

\vspace{1cm}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

==> related.tex <==
\subsection{Related Works}

{\bf NOTE:} Let us list all the papers that we have found useful. A short sentence for each reference in the introduction would be useful for future reference.

\cite{toyoizumi05:BCM}
\cite{habenschuss13:stdp}
\cite{buesing11:sampling}
\cite{kappel15:synaptic}
\cite{quinn15:dig}
\cite{leibfried15:reward}
\cite{klampfl09:ibica}

\vspace{1cm}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

==> supervised.tex <==
\section{Supervised Learning}

\noindent {\bf Classification.} \note{special case for classification with multiple target classes.} Time-series data from time $0$ to $t$ is given as two parts: input $\bfx^t$ and target class $y^t$, where a target class $y \in \{1, \cdots, C\}$ is represented by either (i) one unit of categorical values or (ii) $C$ number of binary units, \ie, $\bfe_y = (1_{k=y})_{k=1}^C$. Then, all the above representations can be applied to the pair of time-series data $\bfx^t, y^t$ (both are visible) as form of $p(\bfx_t, y_t | \bfx^{t-1}, y^{t-1})$. Then, training this model to solve a particular classification problem can be defined in two different way: one is generative objective to maximize $\log p(\bfx^t, y^t)$ and the other is discriminative objective maximize $\log p(y^t | \bfx^t)$.

\note{need to elaborate more..}

\vspace{3cm}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:
